Flow Straight and Fast: Learning to Generate and Transfer Data with Rectified Flow

We present rectified flow, a surprisingly simple approach to learning (neural) ordinary differential equation (ODE) models to transport between two empirically observed distributions \pi_0 and \pi_1, hence providing a unified solution to generative modeling and domain transfer, among various other tasks involving distribution transport. The idea of rectified flow is to learn the ODE to follow the straight paths connecting the points drawn from \pi_0 and \pi_1 as much as possible. This is achieved by solving a straightforward nonlinear least squares optimization problem, which can be easily scaled to large models without introducing extra parameters beyond standard supervised learning. The straight paths are special and preferred because they are the shortest paths between two points, and can be simulated exactly without time discretization and hence yield computationally efficient models. We show that the procedure of learning a rectified flow from data, called rectification, turns an arbitrary coupling of \pi_0 and \pi_1 to a new deterministic coupling with provably non-increasing convex transport costs. In addition, recursively applying rectification allows us to obtain a sequence of flows with increasingly straight paths, which can be simulated accurately with coarse time discretization in the inference phase. In empirical studies, we show that rectified flow performs superbly on image generation, image-to-image translation, and domain adaptation. In particular, on image generation and translation, our method yields nearly straight flows that give high quality results even with a single Euler discretization step.

==> arxiv_textfiles/conclusion.tex <==
\section{Conclusion}


==> arxiv_textfiles/diffusion.tex <==

\section{Connection to Diffusion Models} 
\label{sec:diffusion} 

\subsection{Diffusion Models via Smooth Bridges}
As shown in Section~\ref{sec:marginal}, 
a marginal preserving flow $Z_t$ can be induced from any smooth bridge $X_t$ connecting $\tg_0$ and $\tg_1$. 
By further converting the flow into a diffusion process in a marginal preserving way, we obtain a general  and simple procedure for deriving diffusion models that recovers a large number of existing works. Our procedure highlights the fact that the bridge process $X_t$ (which itself is smooth) and the choice of diffusion coefficient of the learned model can be decoupled as two orthogonal design choices.  

We leverage the following result that has been well exploited the in the literature. 

\begin{pro}
Assume the conditions in Theorem~\ref{thm:marginal}. 
In addition, let $p_{X_t}(z)$ be the shared density function 
of $X_t$ and $Z_t$, which we assume to be 
continuously differentiable and positive everywhere on $\RR^d$. 
Assume $\{U_t\}$ solves the following  stochastic differential equation: %
\bbb\label{equ:Udiff}
\d  U_t = v^{\X,\sigma}(U_t, t)\dt  + \sigma_t \d W_t, && U_0 \sim \tg_0 && \text{with} && 
v^{\X,\sigma}(z,t)= v^\X(z,t) + \frac{\sigma_t^2}{2} \dd \log p_{X_t}(z), 
\eee  
where $\sigma_t \in \RR$ is a positive sequence and $W_t$ is a standard Brownian motion. 
Then  $U_t$ shares the same marginal laws with $Z_t$ (and $X_t$) for all time $t$, that is, $\law(U_t) = \law(Z_t) = \law(X_t)$, $\forall t\in[0,1]$. 
\end{pro}

Therefore, the diffusion process $U_t$ also provides a draw from $U_1\sim \tg_1$ from the target distribution, 
although the resulting coupling $(U_0,U_1)$ is different from $(Z_0,Z_1)$, 
and no longer guarantees to yield lower convex transport costs than $(X_0,X_1)$ %
due to the introduction of the diffusion noise. 

In the following, we discuss two approaches to estimate $v^{\X,\sigma}$: 
one based on modifying the loss function in \eqref{equ:Lgvphi} which recovers the (continuous limit of) training receipts \red{in \cite{song2020denoising, ho2020denoising}}; 
another constructs $v^{\X,\sigma}$ directly from estimates of $v^\X$ without retraining. 

\subsubsection{Training Diffusion Models via Smooth Bridges}

To construct a mean square style  loss function for $v^{\X, \sigma}$, we need to express $\dd \log p_t(x)$ into a conditional expectation of something that can be empirically calculated based on draws of $X_t$. 
This is made possible with the following well known relation (see Lemma~\ref{lem:xydlogp} in \red{Appendix}): 
$$
\dd_x \log p_{X_t}(x) =\E[ \dd_x \log p_{X_t|C_t}(x~|~C_t) ~|~ X_t= x],~~~~~\forall x \in \RR^d,
$$ 
where $C_t$ is any random variable on the same probability space for which the conditioned density function $p_{X_t|C_t}$ and its score function $ \dd_x \log p_{X_t|C_t}$ 
exists.  
In practice, we may choose $C_t = (X_0,X_1)$, or $C_t = X_1$ if $X_0$ has an known elementary distribution that can be explicitly marginalized. 
It is preferred to choose a small $C_t$ since resulting estimator would yield a smaller variance. %

Hence, $v^{\X,\sigma}$ can be expressed into the solution of 
\bbb \label{equ:vctxx} 
\min_{v} \int_0^1 w_t \E\left [ \norm{v(X_t, t) - Y_t}^2_2 \right] \dt, &&
Y_t = \ddtdot X_t + \frac{\sigma_t^2}{2} \dd \log p_{{X_t|C_t}}(X_t~|~C_t), 
\eee
and $v^{\X, \sigma}(x, t) = \E[Y_t~|~X_t = x]$, 
where $w_t>0$ is a positive sequence. 


  

The procedure above provides a  general procedure to constructing denoising diffusion models. 
It allows us to specify the methods via two orthogonal components: 

1) the interpolation curve $X_t$ which serves to specify the sequence $\{\pi_t\}$ of marginal distributions that connect the source $\tg_0$ and target $\tg_1$. 

2) The diffusion coefficient $\sigma_t$ specifying how random we want during the inference time. 

\paragraph{A Recipe 
for Diffusion Models with Gaussian Noise} 
A canonical case of \eqref{equ:vctxx}, 
which covers a number of existing  diffusion models, 
is when 
$X_t$ can be represented into a sum of a random variable with a Gaussian noise. 
Specifically, assume $X_t$ is chosen to have a form of $X_t = \phi_t + \gamma_t \xi$, 
where $\phi_t, \gamma_t$ are differentiable (random) curves  and $\xi \sim \normal(0,I)$ is a standard Gaussian noise that is independent with $C_t \defeq (\phi_t,\gamma_t)$. Then, we have $X_t ~|~ C_t \sim \normal(\phi_t, \gamma_t^2I),$ and hence 
$\dd \log p_{X_t|C_t}(X_t ~|~ C_t) = 
 \gamma_t^{-2}(\phi_t- X_t) = -\gamma_t^{-1} \xi. 
$ 
Following~\ref{equ:vctxx}, this yields 
\bbb \label{equ:ddgauss} 
X_t = \phi_t + \gamma_t \xi, &&
Y_t = \dot \phi_t + \left( \dot \gamma_t  - \frac{\sigma_t^2 }{2\gamma_t} \right) \xi. 
\eee  
Similar procedures can be derived 
 when $\xi$ follows a general distribution with a known density function. 


 
\paragraph{Example: SMLD and DDPM}
The instances of diffusion models in \cite{song2020denoising}, including 
SMLD and DDPM,  can be recovered  using the following choices of $\{X_t\}$ and $\sigma_t$: 
\bb 
X_t = \alpha_t X_1 + \gamma_t \xi, && 
Y_t = \dot \alpha_t X_1 + \left (\dot \gamma_t - \frac{1}{2} \frac{\sigma_t^2}{\gamma_t}\right)  \xi, && 
 {\sigma_t^2} = 2\gamma_t^2  \left (\frac{\dot\alpha_t}{\alpha_t} -\frac{\dot \gamma_t}{\gamma_t} \right ),
\ee 
with $\alpha_t = 1$ for SMLD and $\alpha_t = \sqrt{1-\gamma_t^2}$ for DDPM. 
Note that diffusion coefficient $\sigma_t$
is determined 
by $\alpha_t$ and $\gamma_t$ through the formula, which is a consequence of using O-U process. %
Using the formula in \eqref{equ:ddgauss}, the target $Y_t$ in the loss function is 
$Y_t = \dot \alpha_t X_1 + \left (\dot \gamma_t - \frac{1}{2} \frac{\sigma_t^2}{\gamma_t}\right)  \xi_t,$ which we show is equivalent to these used in DDPM and SMLD; see appendix for the derivation.  
In this case, the initial $X_0$ is defined implicitly, $X_0 = \alpha_0 X_1 + \gamma_0 \xi $, which depends on the final value $X_1$ unless $\alpha_0 = 0$. 
Both SMLD and DDPM assumed that $\alpha_0 /\gamma_0 \approx 0$, so that $X_0$ approximately follows $\normal(0, \gamma_0^2)$, which is set to the source distribution $\tg_0$. 

Further, when $X_t = \alpha_t X_1 + \gamma_t \xi$, we must have 
$X_1 = \alpha_1 X_1 + \gamma_1 \xi$, and hence $
\alpha_t = 1$
 and $\gamma_1 = 0$. 


 \paragraph{Example: Brownian Bridge.} 
If we take $
 X_t = t X_1 + (1-t) X_0 +  \sigma_t \sqrt{t (1-t)} \xi, 
 $
 where $\xi\sim \normal(0,I)$ 
 and $\sigma_t >0$. 
 It can be shown that $\law(X_t)$ coincides with the marginal law of the Brownian bridge $\d U_t = \frac{X_1-U_t}{1-t} \dt + \sigma_t \d W_t$ with $U_0 = X_0$, which is used to construct diffusion models in \red{\citet{bridge}}.  
 We show in Appendix that the $Y_t$ in 
 \eqref{equ:ddgauss} can be reduced to $Y_t = \frac{X_1 - X_t}{1-t}$ (by canceling out $\xi$), 
 which coincides with the velocity field of Brownian bridge $U_t$. 
 
\paragraph{Issue of Variance Exploding} 
Compared with {\name} flow, the training method \red{above} 
has an extra term $\frac{\sigma_t^2}{\gamma_t}$, 
because $\gamma_t$ must go to zero as $t\to 1$,
this term would cause exploding problem unless $\sigma_t$ also decays to zero. 
In fact, the choice of SMLD/DDPM has 
$$
\frac{\sigma_t^2}{2\gamma_t} = \gamma_t \left (\frac{\dot \alpha_t}{\alpha_t} - \frac{\dot \gamma_t}{\gamma_t} \right ). $$
Hence $Y_t = \dot \alpha_t X_1 + \left (2\dot \gamma_t - \gamma_t \frac{\dot \alpha_t}{\alpha_t} \right ) \xi$, which does not seem to explode??? %

However, a typical choice of $w_t$ as suggested by maximum likelihood estimator is $w_t = \sigma_t^{-2}$, which would explode when $\sigma_t \to 0$ as $t\to 1$. 

The balanced choice of $\gamma_t, \sigma_t, w_t$ has been a subject of a number of recent works from both theoretical and empirical angles \red{[cite: Jun Zhu paper, Nvidia paper, etc]}


\subsection{Training-free Conversion between Flow and Diffusion Models} 

Another special property of $X_t$ of form $X_t = \alpha_t X_1 + \gamma_t \xi$ with $\xi \sim \normal(0,I)$ is that the velocity field $v_\sigma^*(x,t)$ 
with any diffusion coefficient $\sigma_t$ can be readily determined from the flow velocity field, without requiring to re-train the model. 
This approach was used in DDIM \red{[]} and  \red{song, sde} to convert a diffusion model to flow (although training with the right target may yield better results). Our derivation suggests that this seems to be a special property of  $X_t = \alpha_t X_1 + \gamma_t \xi$ with Gaussian $\xi$. 


\begin{pro}
Assume $X_t = \alpha_t X_1 + \gamma_t \xi$, where $\alpha_t, \gamma_t \neq 0$ and $\xi \sim \normal(0, I), X_1 \sim \tg_1$. 
For any $\sigma_t >0$ and $v_\sigma^*(x,t)$ in \eqref{equ:Udiff} with $v^*(x,t) = v_0^*(x,t) =  \E[\dot X_t |X_t= x]$,  we have 
$$
v_{\sigma}^*(x,t) = v^*(x,t) + 
\frac{\sigma_t^2}{2\gamma_t^2} \left ( 
a_t v^*(x,t)  - (1+ b_t) x)
\right )
$$
where 
$a_t = \left(\frac{\dot \alpha_t}{\alpha_t} -  \frac{\dot \gamma_t}{\gamma_t} \right )^{-1}$, and 
$b_t =   a_t \frac{\dot \gamma_t}{\gamma_t},$ provided that $a_t, b_t$ are finite $\forall t\in (0,1)$.   
\end{pro}
Note that $c_t = \gamma_t^2$ when we take $\sigma_t^2 = 2 \gamma_t^2 \left(\frac{\dot \alpha_t}{\alpha_t} -  \frac{\dot \gamma_t}{\gamma_t} \right )$ as the case of SMLD and DDPM. 

Hence, if we already have trained a model $\hat v \approx v^*$ for the flow. 
Could we directly  construct a diffusion model directly from $\hat v_\sigma = a_t \hat v - b_tx$ for any $\sigma_t$ without retraining. 

\paragraph{Example: Rectified flow to Diffusion} 
Assume $X_t = t X_1 + (1-t)X_0$, and $X_0 \sim \normal(0,  \beta_0^2I).$   Then we have $\alpha_t = t$ and $\gamma_t = \beta_0 (1-t)$, and hence 
\bb  
a_t = \frac{1}{2}\left ( \frac{1}{t} + 
\frac{1}{1-t}\right )^{-1} = \frac{1}{2} {t(1-t)}, &&
b_t =  -\frac{1}{2} {t(1-t)} \frac{1}{1-t} = 
-\frac{1}{2} t. 
\ee 
Hence 
$$
v_\sigma^*(x,t) =
v^*(x,t) + 
\frac{\sigma_t^2}{2 \beta_0^2(1-t)^2}  
\left ( \frac{t(1-t)}{2} v^*(x,t) - \frac{2-t}{2} x \right ).
$$
If we follow the choice of $\sigma_t^2$ in DDPM/SMLD, 
we have $\sigma_t^2 = 2\beta_0^2\frac{1-t}{t}$. 

But maybe we should take $\sigma_t^2 = \beta_0^2 (1-t)^2$ instead... 

\begin{proof} 
Assume $X_t = \alpha_t X_1 + \gamma_t \xi$. In this case, $p_t(x) \propto \E_{X_1}\left [ \exp \left (-\frac{\norm{X_t - \alpha_t X_1}^2}{2\gamma_t^2} \right )~|~ X_t =x \right ]$, and 
$$
\dd \log p_t(x) =  \frac{1}{\gamma_t^2} \E[\alpha_t X_1 - X_t | X_t = x] = 
\frac{1}{\gamma_t^2}(\alpha_t \E[X_1|X_t=x] - x). 
$$
On the other hand, 
\bb 
v^*(x,t) 
& = \E[\dot \alpha_t X_1 + \dot \gamma_t \xi ~|~ X_t = x] \\ 
& =  \E\left [\dot \alpha_t X_1 +
\frac{\dot \gamma_t}{\gamma_t} (X_t - \alpha_t X_1 ) ~|~ X_t = x \right ]  \\
& = 
\left(\dot \alpha_t -  \alpha_t \frac{\dot \gamma_t}{\gamma_t} \right ) \E[X_1|X_t =x]  + \frac{\dot \gamma_t}{\gamma_t} x
\ee 
Hence 
$$
\dd \log p_t(x) = \frac{1}{\gamma_t^2} \E[\alpha_t X_1 - X_t | X_t = x] =
\frac{1}{\gamma_t^2} 
\left(\frac{\dot \alpha_t}{\alpha_t} -  \frac{\dot \gamma_t}{\gamma_t} \right )^{-1} \left ( v^*(x,t) -   \frac{\dot \gamma_t}{\gamma_t} x 
\right ) - \frac{1}{\gamma_t^2} x. 
$$
Hence 
\bb 
v_\sigma^*(x,t) 
& = v^*(x,t) + 
\frac{\sigma_t^2}{2\gamma_t^2}\left(\frac{\dot \alpha_t}{\alpha_t} -  \frac{\dot \gamma_t}{\gamma_t} \right )^{-1} \left ( v^*(x,t) -  \frac{\dot \gamma_t}{\gamma_t} x 
\right ) - \frac{\sigma_t^2}{2\gamma_t^2} x \\ 
& =  a_t v^*(x,t) - b_t x, 
\ee 
where 
\bb 
a_t = 1 + \frac{\sigma_t^2}{2\gamma_t^2}\left(\frac{\dot \alpha_t}{\alpha_t} -  \frac{\dot \gamma_t}{\gamma_t} \right )^{-1} , 
&&
b_t =   \frac{\sigma_t^2}{2\gamma_t^2} + \frac{\sigma_t^2}{2\gamma_t^2}\left(\frac{\dot \alpha_t}{\alpha_t} -  \frac{\dot \gamma_t}{\gamma_t} \right )^{-1} \frac{\dot \gamma_t}{\gamma_t}
\ee 
Note that if we take $\sigma_t^2 = 2 \gamma_t^2\left(\frac{\dot \alpha_t}{\alpha_t} -  \frac{\dot \gamma_t}{\gamma_t} \right )$ as SMLD and DDPM, %
we have 
\bb 
a_t = 2, %
&&
b_t =  \frac{\sigma_t^2}{2\gamma_t^2}  + \frac{\dot \gamma_t}{\gamma_t} = \frac{\dot \alpha_t}{\alpha_t}. 
\ee
\end{proof} 

\subsection{Why Should we use Diffusion Noise?} 

\section{Generalization to Diffusion Models}

\trash{Question: what is the benefit of diffusion? Or is it not useful at all?}

Further generalization of our  approach to allow $X_t$ to be a random, non-smooth curve that connect $X_0$ with $X_1$ (called bridge processes), 
such a framework is considered in \red{[], [].}

Our earlier result can be viewed as a special case. 

In particular, 
assume $X_t$ is a stochastic  process that satisfies $\d X_t = b(X_t, t) \dt + \sigma_t(X_t,t) \d W_t$ that satisfies $X_0 \sim \tg_0$ and $X_1 \sim \tg_1$. 
We call it a stochastic bridge. 

\begin{pro}
Assume $\d X_t = b(X,t) \dt  + \sigma(X, t) \d W_t$. Then the following SDE shares the same marginal distribution: 
\bbb \label{equ:zdiffusion}
\d Z_t = \bar v(X_t, t) \dt + \bar \sigma (X_t, t) \d W_t,
\eee 
where 
\bbb \label{equ:condivb}
\bar v(x,t) = \E[b(X,t)~|~X_t = x],
&& 
\bar \sigma^2(x,t) = \E[\sigma^2(X,t)~|~X_t = x],
\eee 
where $\sigma^2 = \sigma\sigma\tt$ if $\sigma$ is matrix.
Assume $Z_t$ is the unique solution of \eqref{equ:zdiffusion} and $\law(Z_0) = \law(X_0)$. 
Then $\law(Z_t) = \law(Z_t)$ for every $t \geq 0$. 
\end{pro}
\begin{proof}
Let $h$ be a compactly supported continuously differentiable test function, we have by Ito's lemma: 
\bb 
\ddt  \E[h(X_t)] 
& = \E\left [\dd h(X_t) \tt b(X,t)  + \frac{1}{2} \trace(\dd ^2 h(X_t) \sigma^2(X,t)) \right ] \\
& = \E \left [ \dd h(X_t) \bar b(X_t,t) + \frac{1}{2} \trace(\dd^2 h(X_t) \bar \sigma^2(X_t,t) ) \right ] \ant{following \eqref{equ:condivb}}. 
\ee 
This suggests the marginal distribution $\pi_t$ of $X_t$ follows the Fokker Planck (FP) equation in the distributional \red{weak?} sense: 
$$
\ddtdot \pi_t + \div(\bar v_t \pi_t )  - \frac{1}{2} \Delta \pi_t = 0. 
$$
But the marginal distribution of $Z_t$ follows the same FP equation with the same initialization.  The result then follows the uniqueness of the solution. 
\end{proof}

\paragraph{A Practical Recipe for Diffusion Models}
A key challenge in designing such algorithms is to specify bridge processes that satisfy the end point conditions. 
\red{[]} introduced several methods to achieve this. 
It is mainly based on specifying the SDE, and then derive the solution. Here we directly specify the solution. 
Let $X_t$ has a form of 
$$
X_t = \phi(X_1, X_0,t) + \gamma_t \xi_t,
$$
where $\xi_t \sim \normal(0,I_d)$  and $\gamma_t$ is a sequence that satisfies $\gamma_t \geq 0$ and $\gamma_1 = 0$, and $\phi(X_1,X_0, 1) = X_1$.  
We do not necessarily require that $\gamma_0 = 0$, and $\phi(X_1,X_0,0)=X_0$.   
So $Z_t$ is any sequence of random variables that satisfies $Z_1 = X_1$. 

In addition, we specify a sequence $\sigma_t\geq0$ which is the diffusion coefficient of the learned model. The learned generative process is then 
\bb 
\d Z_t = f(Z_t, t) \dt + \sigma_t \d W_t,
&& Z_0 \sim \phi(X_1, X_0,0) +  \gamma_0 \xi_0,
\ee 
and the loss function is 
\bbb \label{equ:diffloss}
\min_{v} \int_0^1 \E [w_t \norm{v(Z_t, t) - Y_t}_2^2 ],
\eee 
where $Y_t = \partial_t \phi(X_1,X_0, t) - \frac{\sigma_t^2}{2 \gamma_t} \xi_t,$
 and $w_t$ is a set of positive weights as used in typical denoising diffusion models. 

\begin{thm}
Assume $X_t = \phi(X_0,X_1,t) + \gamma_t \xi_t$, $t\in[0,1]$,  where $\phi_t$ and $\gamma_t$ are a continuously differentiable process and $\gamma_t\geq0$, and 
$\xi_t$ is any stochastic process that satisfies $\law(\xi_t)=\normal(0,I),~\forall t$. 
Assume $Z_t$ is the unique solution of $\d Z_t = v^*(Z_t,t) \dt + \sigma_t \d W_t$, where 
$v^*(z,t) = \E[ \partial_t \phi(X_0,X_1, t) +  (\dot \gamma_t - \frac{1}{2}\frac{\sigma_t^2}{\gamma_t} )\xi_t ~|~ X_t = x]$, and 
$W_t$ is a standard Brownian motion, and $\sigma_t\geq0$. 
Then $\law(Z_t) = \law (X_t)$ for $ \forall t\in[0,1]$.  
\end{thm}

Note that when setting $\sigma_t =0$, it is a straightforward generalization of the deterministic version when $X_t = \phi(X_1,X_0,t)$. The KL divergence minimization advises that we should take $w_t = \sigma_t^2$. But alternative choices can also be good. In particular, one choice is variance balance one that takes $w_t = 1/\var(Y_t)^2$. 



So we can see that the introduction of $\xi_t$ allows us to allocate part of randomness to the process, rather than pushing all randomness to the initialization. 

we just need to find an oracle diffusion process whose marginals match that of $Z_t$, and then construct a loss function to approximate it. 



 \paragraph{Example: Brownian Bridge.} 
If we take $
 X_t = t X_1 + (1-t) X_0 +  \sigma_t \sqrt{t (1-t)} \xi_t, 
 $
 where $\sigma_t >0$. It can be shown that there exists a stochastic process $\xi_t$ with $\law(\xi_t) = \normal(0,I)$, such that $X_t$ is the solution of $\d X_t = \frac{X_1-X_t}{1-t} \dt + \sigma_t \d W_t$, which is the Brownian bridge (when $\sigma_t=1$); see \red{\citet{bridge}}. 
  It can be shown that in this case $\vofX(x,t) = 
  \E[Y_t~|~X_t = x] = \E[\frac{X_1 - X_t}{1-t} ~|~ X_t=x]$.  

 
\paragraph{Example: SMLD and DDPM}
SMLD and DDPM can be viewed as taking $X_t = \alpha_t X_1 + \gamma_t \xi_t$ with $\alpha_t = 1$ for SMLD and $\alpha_t = \sqrt{1-\gamma_t^2}$ for DDPM, and setting the diffusion coefficient to be  $ {\sigma_t^2} = 2\gamma_t^2  (\frac{\dot\alpha_t}{\alpha_t} -\frac{\dot \gamma_t}{\gamma_t})$ (which means that $\alpha_t,\gamma_t$ should be constructed to satisfy  $\frac{\dot\alpha_t}{\alpha_t} -\frac{\dot \gamma_t}{\gamma_t}\geq 0$). 
Using our formula, the target $Y_t$ in the loss function should be 
$Y_t = \dot \alpha_t X_1 + \left (\dot \gamma_t - \frac{1}{2} \frac{\sigma_t^2}{\gamma_t}\right)  \xi_t.$ 
See appendix for the derivation. 

We should note that in both SMLD and DDPM, 
the $X_0$ only follows the assumed $\tg_0$ approximately.  
In SMLD, it is assumed that $X_t = X_1 + \gamma_t \xi_t$ and hence $X_0 = X_1 + \gamma_0 \xi_0$, which depends on $X_1$. SMLD assumes that $\gamma_0$ is sufficiently large so that $X_0$ approximately follows $\normal(0, \sigma_0I)$. 
In DDPM, we have $X_t =\alpha_t X_1 + \gamma_t \xi_t$, and it is assumed that $\alpha_t$ is very close to zero, so that $X_0 = \alpha_0 X_1 + \gamma_t \xi_t$ approximately follows $\normal(0, \gamma_t I)$. In the light of  our general formula, there is no reason to not set $\alpha_0=0$ to get an exact initial condition. This issue is also discussed in \red{\citet{bridge}\citet{peluchetti2021non}}. 

 \subsection{The choice of $\sigma_t$ and $\gamma_t$?}
 
 If $\sigma_t=0$, it reduces to \red{mixupflow} 
 if we treat $\gamma_t \xi_t$ as a part of the random from $\tg_0$.
 
 One tricky issue with introducing the diffusion 
 noise is that 

So we then have $X_t = \phi_t + \gamma_t \xi_t$, and $Y_t = \dot \phi_t + (\dot \gamma_t - \frac{1}{2}\frac{\sigma_t^2}{\gamma_t} ) \xi_t$. 

Note that $\gamma_t$ has to decrease to zero when $t\to 1$, which causes the variance to explode as $t\to 1$. In addition, there is further complication  in choosing the importance weight. Using MLE, we need to choose $w_t = 1/\sigma_t^2$, this means that $\sigma_t$ decaying to zero would causes problem.  


1) It seems that one possibility is to decay $\sigma_t$ and $\gamma_t$ together to zero, and ensure that $\dot \sigma_t$ is bounded, and use uniform weights $w_t = 1$. 


\subsection{Proof of the Flow to Diffusion Conversion}
Recall that the marginal law $\pi_t \defeq  \law(Z_t)=\law(X_t)$ follows $\ddtdot \pi_t + \div (\vofX_t \pi_t) = 0$. 

This is equivalent to 
$\ddtdot \pi_t + \div( (\vofX_t + \frac{1}{2 } 
\frac{\dd(\sigma^2_t \pi_t) }{\pi_t}) \pi_t) - \frac{1}{2} \Delta (\sigma^2_t \pi_t) = 0$. 

Hence the following  $
\d Z_t = 
\left (v^*(Z_t,t) + \frac{1}{2 } 
\frac{\dd(\sigma^2_t(Z_t,t) \pi_t(Z_t)) }{\pi_t})  \right )\dt + \sigma_t(Z_t,t)\d W_t
$. 

In fact, 
$\d Z_t = \left (v^*(Z_t,t) + \frac{1}{2 } 
\frac{\dd(\sigma^2_t(Z_t,t) \pi_t(Z_t)) }{\pi_t})  \right )\dt + \sigma_t(Z_t,t)\d W_t$. 
Hence, we want to set the target $Y_t$. 
$$
Y_t = \ddtdot X_t + \frac{1}{2} \sigma_t^2 \dd_{X_t} \log  \pi_t(X_t~|~ X_0,X_1). 
$$

We can take 
$$
Y_t = \ddtdot X_t + \frac{1}{2} \sigma_t^2 R_t, 
$$
where $R_t$ is any random number that satisfies $\E[R_t~
|~X_t = x] = \dd_{x} \log \pi_t(x)$. 


\subsection{Appendix: SMLD and DDPM}



\paragraph{Connection to SMLD}  
 SMLD \citep{song2019generative, song2020score, song2020denoising} assumes $X_t$ is a Brownian motion backward in time, that is, $X_t = \rev X_{1-t}$ and $\d \tilde X_t = \sigma_{1-t}\d W_t$. By the time reversal formula, this is equivalent to $\d X_t = \sigma_t^2 \frac{X_1 - X_t}{\gamma_t^2} \dt + \sigma_t \d W_t$, where $\gamma_{t}^2 = \int_{t}^1 \sigma_{s}^2 \d s$ and hence $\sigma_t^2 = - 2\gamma_t \dot \gamma_t$. 
 
Using our approach, we note that $\d \tilde X_t = \sigma_{1-t}\d W_t$ implies that $X_t = X_1 + \gamma_t \xi_t$. %
 Hence 
 $$Y_t =
 \left (\dot \gamma_t -\frac{1}{2} \frac{\sigma_t^2}{\gamma_t} \right )\xi_t = 
 \frac{\sigma_t^2}{\gamma_t^2} (X_1- X_t), 
 $$
 which matches the time reversal formula. 
 
\paragraph{Connection to DDPM}   
DDPM \citep{ho2020denoising} assumes that the time-reversed process $\rev X_t = X_{1-t}$ satisfies 
$\d \rev X_t = \eta_{1-t} \rev X_t \dt + \sigma_{1-t} \d W_t$,
It solution is 
\bb 
X_t = \alpha_t X_1 +
\gamma_t \xi_t,  && \alpha_t = \exp\left(\int_t^1 \eta_s \d s \right), && 
\gamma_t^2 = \int_t^1 \exp\left (2\int_t^s \eta_r \d r \right)  \sigma_{s}^2 \d s.  
\ee 
The time-reversion formula gives 
\bbb \label{equ:xtddpm} 
\d X_t = \left(- \eta_{t} X_t + \sigma_t^2 
\frac{\alpha_t X_1 - X_t }{\gamma_t^2}\right )\dt + \sigma_t \d W_t.
\eee  
Using our formula \red{[xxx]}, 
the regression target should be $Y_t  = \dot \alpha_t X_1 + \left (\dot \gamma_t - \frac{1}{2} \frac{\sigma_t^2}{\gamma_t}\right)  \xi_t$. 
To see that this is consistent with \eqref{equ:xtddpm}, note that by the definition of $\alpha_t, \gamma_t$ above, we have 
\bb 
\eta_t = -\frac{\dot \alpha_t}{\alpha_t}, && 
2\gamma_t\dot \gamma_t = -\sigma_t^2 -2 \gamma_t^2 \eta_t, 
\ee  
or $\frac{\dot \gamma_t}{\gamma_t} =  - \frac{\sigma_t^2}{2\gamma_t^2} +  \frac{\dot\alpha_t}{\alpha_t}.$ Hence 
\bb 
Y_t 
& = \dot \alpha_t X_1 + \left (\dot \gamma_t - \frac{1}{2} \frac{\sigma_t^2}{\gamma_t}\right)  \xi_t \\
& = \dot \alpha_t X_1 + \left (\frac{\dot \gamma_t}{\gamma_t} - \frac{1}{2} \frac{\sigma_t^2}{\gamma_t^2}\right) (X_t - \alpha_t X_1) \\
& 
= \dot \alpha_t X_1 + \left (\frac{\dot \alpha_t}{\alpha_t} -  \frac{\sigma_t^2}{\gamma_t^2}\right) (X_t - \alpha_t X_1) \\
& =
 -\eta_t 
 X_t + 
\frac{\sigma_t^2}{\gamma_t^2}\right) (
\alpha_t X_1 - X_t), 
\ee 
which reduces to \eqref{equ:xtddpm}. 


 

 


\subsection{Derivation of diffusion case}
Assume $X_t = \phi(X_1, X_0, t) + \alpha_t W_{ \beta_t} $, 
where $W_t$ is a standard Brownian motion. 
Note that $\d W_{\beta_t} =  \dot \beta_t^{1/2} \d \tilde W_{t}$. 
Taking gradient: \bb 
\ddtdot X_t 
& = \ppt \phi(X_1, X_0, t) + \dot \alpha_t W_{\beta_t} + \alpha_t \d W_{\beta_t}  \\
&  = \ppt \phi(X_1, X_0, t) + \dot \alpha_t W_{\beta_t} + \alpha_t \dot \beta_t^{1/2} \d W_t . 
\ee 
We hope that $\sigma_t = \alpha_t \dot \beta_t^{1/2},$
and the variance of the diffusion term is 
 $\gamma_t^2 =\alpha_t^2 \beta_t.$
 $$
 s_t^2 = \var(\dot \alpha_t W_{\beta_t}) 
 = \int \dot \alpha_t 
 $$
 We want to represent $s_t$ using $\sigma_t$ and $\gamma_t$. 
 
 \begin{lem}
 Assume $X_t = \phi_t + \alpha_t W_{\beta_t}$, where $\phi_t, \alpha_t, \beta_t$  are $C^1$ sequences and $\alpha_t, \beta_t$ are non-negative. 
 
 Then $X_t$ follows
 \bb 
 \d X_t 
 & = (\dot \phi_t  + \dot \alpha_t W_{\beta_t})\dt +  \alpha_t \d W_{\beta_t} \\ 
 & = \left (\dot \phi_t + \frac{\dot \alpha_t}{\alpha_t} \left(X_t - \phi_t\right)\right) \dt   + \alpha_t \dot \beta_t^{1/2} \d \tilde W_t,
\ee 
where $\tilde W_t$ is defined by $\beta_t^{1/2} \d \tilde W_t = \d W_{\beta_t}$, and it is a standard Brownian motion. 

Let $\gamma_t = \alpha_t \beta_t^{1/2}$, and $\xi_t \sim \normal(0, I)$, then  $\gamma_t  \xi_t \deq \alpha_t W_{\beta_t}$, and  then $X_t = \phi_t + \gamma_t \xi_t $. 

Following Lemma~\ref{lem:abc} below, the drift term $Y_t$ is 
\bb 
 Y_t
& = \dot \phi_t  + \dot \alpha_t W_{\beta_t} \\ 
& = \dot \phi_t + \frac{\dot \alpha_t }{\alpha_t } \alpha_t W_{\beta_t}  \\ 
& = \dot \phi_t + \frac{\dot \alpha_t }{\alpha_t } \gamma_t \xi_t  \\
&= \dot \phi_t + s_t \xi_t \\
& = \dot \phi_t + \left (\dot \gamma_t - \frac{1}{2}\frac{\sigma_t^2}{\gamma_t}\right ) \xi_t. 
\ee 
 \end{lem}
 
 
 \begin{lem}\label{lem:abc}
 Assume 
 \bb
 \sigma_t^2 = \alpha_t^2 \dot \beta_t , &&
 \gamma_t^2 = \alpha_t^2 \beta_t, &&
 s_t^2 = \dot \alpha_t^2 \beta_t.
 \ee 
 Then 
 \bb 
 s_t = \dot \gamma_t  - \frac{1}{2} \frac{\sigma_t^2}{\gamma_t},  &&  
 \frac{\dot \alpha_t}{\alpha_t} =\frac{s_t}{\gamma_t} = \frac{\dot \gamma_t}{\gamma_t} - \frac{1}{2} \frac{\sigma_t^2}{\gamma_t^2}. 
 \ee 
 \end{lem}
 \begin{proof}
 \bb \dot \gamma_t =  \dot \alpha_t \beta_t^{1/2} + \frac{1}{2}\alpha_t \beta_t^{-1/2} \dot \beta_t 
 = s_t + \frac{1}{2} \frac{\sigma_t^2}{\gamma_t}.  
 \ee 
 \bb
 \frac{\dot \alpha_t}{\alpha_t} =\frac{s_t}{\gamma_t} 
 = \frac{\dot \gamma_t}{\gamma_t} - \frac{1}{2} \frac{\sigma_t^2}{\gamma_t^2}. 
 \ee 
 \end{proof}
 

 \paragraph{Example: Brownian Bridge (Derivation).} 
 Assume 
 $$
 X_t = t X_1 + (1-t) X_0 + \sigma_t \sqrt{t (1-t)} \xi_t,
 $$
 where $\sigma_t>0$. Then 
 \bb 
 Y_t 
 & = (X_1 - X_0) + \left(\sigma_t \frac{1-2t}{2\sqrt{t(1-t)}} -\frac{\sigma_t}{2 \sqrt{t(1-t)}}  \right) \xi_t  \\
 & = (X_1 - X_0) - \sigma_t \frac{\sqrt{t}}{\sqrt{1-t}} \xi_t \\
 & = (X_1 - X_0)  -  \frac{\sqrt{t}}{\sqrt{1-t}} \frac{X_t - t X_1 - (1-t) X_0}{\sqrt{t(1-t)}} \\
 & = (X_1 - X_0)  -  \frac{{1}}{{1-t}} ({X_t - t X_1 - (1-t) X_0}) \\
 & = \frac{X_1 - X_t}{1-t}. 
 \ee 
 This matches the updates of Brownian motion. 
 This matches the updates of Brownian motion. 
 

\section{planer}

\trash{ 
\paragraph{Generalization: Random Hitting Time}
Set $X_t = \Phi(X_1, X_0, t)$ and $\tau_t = \Psi(X_0, X_1, t)$, such that $\tau_0 = 0$ and $\tau_t$ is an increasing function. Then try to fit 

$$
\int_0^1 \E[ w_t \norm{ f(Z_t, \tau_t)  - \partial_t [\Phi(X_1, X_0, t); \Psi(X_0, X_1, t)]}_2^2]. 
$$
} 

\begin{enumerate}
    \item \textbf{Generative Models} When $\Pi_0$ is a simple distribution such as Gaussian or uniform distribution, and $\pib$ is observed through a set of data points, this yields a continuous normalizing flow generative model. 
    
    This is our first work, 
    we plan to verify,
    \begin{enumerate}
        \item (Model) Replace diffusion model with ODE, do we observe performance drop? If not, we simplify the current framework.
        \item (Architecture) Currently we do not focus on this.
        \item (Initialization) Design initial transport.
        \item (Training) Inject noise to gradient for large batch size training. %
    \end{enumerate}
    We should show these points from different perspective,
    \begin{enumerate}
        \item (Visually) 2d toys.
        \item (Quantitatively) Image generation. As the first step, to do a quick start, we can start from provided checkpoint. 
    \end{enumerate}
    \item \textbf{CycleGAN, Domain Transfer} When both $\pia$ and $\pib$ are observed through empirical data, this yields a cyclgan like setting. It can potentially used for multimodal generation, such as text to image convertion. 
    \begin{enumerate}
        \item \red{Experiment Idea: Brainstorm} CG prefers to discuss this as a section in a main work, and then create a followup in NLP / Graphics.
        \item text to image transfer?
        \item Translation?
        \item Find typical problem settings of CycleGAN?
    \end{enumerate}    
    \item \textbf{Improving an existing GAN model} 
When $\Pi_0$ is the output of GAN, it allows us to refine the results of GAN using a flow model. 
Further, we can even use this approach to jointly update GAN and the flow by updating the GAN model to amortizing the flow (using the flow direction at time zero to update $\Pi_0$
    \begin{enumerate}
        \item \red{Experiment Idea: Brainstorm} 
    \end{enumerate}
\item \textbf{Autoencoder} 
By amorting both directions of the flow we can get a bidirectional mapping between $\pia$ and $\pib$. 
Because ODE is deterministic, the amortizing would be efficient (amortizing diffusion models can be more challenging). 

    
    As the second work, we need to emphasize different specific points and attract readers. I feel like we can,
    \begin{enumerate}
        \item (Outline) 1. Propose our framework, 2. show one case, 3. leave others as discussions.
        \item (Vision, Better Visualization) When the initial distribution is an auto-regressive model, we hope to improve VQ-GAN works. \emph{This should be the main work.}
        \item (NLG) The experiments take fewer time. \emph{This can be a followup work.}
        \item (Experiment Note) We can start from others' checkpoints. 
        
    \end{enumerate}
\item \textbf{Optimal transport} 
This seems to enable an approximate optimal transport without requiring matching (even though using matching can further improve the result). 
    \begin{enumerate}
        \item \red{Experiment Idea: Brainstorm}
    \end{enumerate}
\item \textbf{Neural ODE / flow } 
This is allows us to learn flow based models without requiring Jacobian computation, or inference (which is already achieved by diffusion models in some sense though).
    \begin{enumerate}
        \item \red{Experiment Idea: Brainstorm}
    \end{enumerate}

\end{enumerate}

 \paragraph{Ablation studies \& Questions to study}
\begin{enumerate}
    \item What is the effect of alpha and beta sequence? 
    \item What is the role of variance exploding? 
    \item What is the role of overfitting? 
    \item How to improve batch size? 
    \item We can generate the method to add diffusion model; what is the effect of diffusion models? Any benefit?
    \item 
\end{enumerate}

 

==> def.tex <==

%----------loading packages------------------
\usepackage{amsmath, amsthm, amssymb, amsfonts, mathtools, graphicx, enumerate}
\usepackage{adjustbox}
\usepackage[utf8]{inputenc} 
\usepackage[T1]{fontenc}    
\usepackage{url}            
\usepackage{booktabs}
\usepackage{nicefrac}       
\usepackage{microtype}      
\usepackage{xspace}
\usepackage{algorithm,algorithmic}
\usepackage{color}
\usepackage{enumitem}
\usepackage{comment}
\usepackage{bm}
\usepackage{apptools}
\usepackage[page, header]{appendix}
\usepackage{titletoc}
\usepackage{array}



\usepackage[scaled=.9]{helvet}

\usepackage{url}
\usepackage{caption}
\usepackage[table,dvipsnames]{xcolor}
\usepackage[colorlinks=true, linkcolor=blue, citecolor=blue]{hyperref}


\usepackage{natbib}
\bibliographystyle{plainnat}
\bibpunct{(}{)}{;}{a}{,}{,}


%----used for show labels
%\usepackage[inner, left]{showlabels}



\newcommand{\theHalgorithm}{\arabic{algorithm}}


\usepackage{amsthm}   
\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}[thm]{Corollary}
\newtheorem{lem}[thm]{Lemma} 
\newtheorem{mydef}[thm]{Definition} 
\newtheorem{ass}[thm]{Assumption} 
\newtheorem{exa}[thm]{Example} 
\newtheorem{rmk}[thm]{Remark} 
\newtheorem{pro}[thm]{Proposition}    % Setting theorem environment 
% fix the spacing problem of theorem
\begingroup
    \makeatletter
    \@for\theoremstyle:=definition,remark,plain\do{%
        \expandafter\g@addto@macro\csname th@\theoremstyle\endcsname{%
            \addtolength\thm@preskip\parskip
            }%
        }
\endgroup





%%%%%%%%%%%%%  COMMON  %%%%%%%%%%%%
\newcommand{\myf}[2]{\frac{\displaystyle #1}{\displaystyle #2}}
 \newcommand{\myp}[2]{\frac{\displaystyle \partial #1}{\displaystyle \partial  #2}}
 \newcommand{\myb}[1]{\mbox{\boldmath$#1$}}
 \newcommand{\eqnref}[1]{Eqn.~\eqref{#1}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\Qiang}[1]{\textcolor{red}{#1}\\}
\newcommand{\qiang}[1]{\textcolor{red}{#1}}
\newcommand{\Todo}[1]{\textcolor{red}{TODO: #1}\\}
\newcommand{\todo}[1]{\textcolor{gray}{TODO: #1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\med}[1]{\textcolor{magenta}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\gray}[1]{\textcolor{gray}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newcommand{\myempty}[1]{}

\newcommand{\ant}[1]{~~~~~~~\text{\med{//#1}}}

\newcommand{\X}{\mathcal{X}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\V}{\mathbb{V}}
\newcommand{\M}{\mathbb{M}}
\newcommand{\HH}{\mathcal{H}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\Z}{\mathcal{Z}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\R}{\mathbb{R}}
%\newcommand{\K}{{\funcset{B}_k}}
\newcommand{\K}{\funcset{K}}%{\funcset{B}_k}}

\newcommand{\A}{\mathbb{A}}

\renewcommand{\S}{\mathbb{S}}

\newcommand{\vx}{\boldsymbol{x}}
\newcommand{\vv}[1]{\boldsymbol{#1}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\RR}{\mathbb{R}}
\newcommand{\neib}[1]{\partial{#1}}
\newcommand{\normal}{\mathcal{N}}
\newcommand{\var}{\mathrm{var}}
\newcommand{\cov}{\mathrm{cov}}
\newcommand{\KL}{\mathrm{KL}}

\newcommand{\Remark}{\paragraph{Remark}}
\newcommand{\remark}{\paragraph{Remark}}


\newcommand{\trace}{\mathrm{trace}}
\newcommand{\diag}{\mathrm{diag}}


\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}

%%%%%%%%%%%%%% Big O notation %%%%%%%%%%%%%%
\newcommand{\op}{o_p}
\newcommand{\Op}{O_p}

\newcommand{\od}{o}
\newcommand{\Od}{O}

\newcommand{\stein}{{\mathcal A}}


\newcommand{\ind}{\mathbb{I}}
\newcommand{\sign}{\mathrm{sign}}

\newcommand{\prob}{\mathrm{Pr}}

\newcommand{\score}{{\vv s}}


\newcommand{\cd}{\mid}


\renewcommand{\k}{{k}}

\newcommand{\kp}{{\mathcal K_p}}
\newcommand{\kpp}{{\mathcal K_{p+}}}

\newcommand{\Kmatrix}{\vv{K}}


%\newcommand{\l}{\left} 
%\newcommand{\r}{\right} 

\renewcommand{\R}{\mathcal{R}}
\newcommand{\aseq}{=}%\overset{\text{\tiny{a.s.}}}{=}}


\newcommand{\yihao}[1]{\textcolor{blue}{ #1}}
\newcommand{\tongzheng}[1]{\textcolor{green}{[TZ: #1]}}
\newcommand{\yrm}[1]{}
\newcommand{\cP}{\mathcal{P}}




\newcommand{\Dset}{\D}
\newcommand{\Sset}{\mathcal{S}}
\newcommand{\Aset}{\mathcal{A}}
\newcommand{\Rset}{\mathbb{R}}
\newcommand{\Pset}{\mathcal{P}}
\newcommand{\mt}{{\operatorname{T}}}
\newcommand{\mi}{{-1}}
\newcommand{\defeq}{:=}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\abs}[1]{\left|#1\right|}

\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\thmref}[1]{Theorem~\ref{#1}}
\newcommand{\corref}[1]{Corollary~\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}


\newcommand{\thetaTD}{\hat{\theta}_{\operatorname{TD}}}
\newcommand{\sbar}{\bar{s}}
\newcommand{\abar}{\bar{a}}
\newcommand{\wb}{\pmb{w}}
\newcommand{\pv}{\rho}

\newcommand{\Fset}{\mathcal{F}}

\newcommand{\qiangremoved}[1]{}
\newcommand{\qq}[1]{\textcolor{red}{\tiny \text{#1}}}

\newcommand{\Kf}{K_0}





\newcommand{\Lrg}{L_{\operatorname{RG}}}
\newcommand{\Lrghat}{\hat{L}_{\operatorname{RG}}}
\newcommand{\Lfvi}{L_{\operatorname{FVI}}}
\newcommand{\Lfvihat}{\hat{L}_{\operatorname{FVI}}}
\newcommand{\Lk}{L_{\k}}
\newcommand{\Lkhat}{\hat{L}_{\k}}
\newcommand{\Lktilde}{\tilde{L}_{\k}}
\renewcommand{\Lk}{L}
\newcommand{\Lktrue}{L^*}

\newcommand{\ellpiq}{\ell_q}

 \def\bb#1\ee{\begin{align*}#1\end{align*}}

 \def\bba#1\eea{\begin{align}#1\end{align}}

\newcommand{\dno}{\mathrm{d}}



\newcommand{\set}[1]{\mathcal{#1}}%\uppercase{#1}}%\mathsf}%{\mathcal}
\newcommand{\funcset}{\mathcal}%\mathfrak}
\newcommand{\dist}[1]{\mathsf{\uppercase{#1}}}%\uppercase}%{\mathsf}%\mathbb} 
\newcommand{\emp}[1]{\hat{\dist{#1}}}
\newcommand{\opt}[1]{{\mathbf{#1}}}



